Enhancing Unsupervised Video Representation Learning by Decoupling the Scene and the Motion

One significant factor we expect the video representation learning to capture, especially in contrast with the image representation learning, is the object motion. However, we found that in the current mainstream video datasets, some action categories are highly related with the scene where the action happens, making the model tend to degrade to a solution where only the scene information is encoded. For example, a trained model may predict a video as playing football simply because it sees the field, neglecting that the subject is dancing as a cheerleader on the field. This is against our original intention towards the video representation learning and may bring scene bias on different dataset that can not be ignored. In order to tackle this problem, we propose to decouple the scene and the motion (DSM) with two simple operations, so that the model attention towards the motion information is better paid. Specifically, we construct a positive clip and a negative clip for each video. Compared to the original video, the positive/negative is motion-untouched/broken but scene-broken/untouched by Spatial Local Disturbance and Temporal Local Disturbance. Our objective is to pull the positive closer while pushing the negative farther to the original clip in the latent space. In this way, the impact of the scene is weakened while the temporal sensitivity of the network is further enhanced. We conduct experiments on two tasks with various backbones and different pre-training datasets, and find that our method surpass the SOTA methods with a remarkable 8.1% and 8.8% improvement towards action recognition task on the UCF101 and HMDB51 datasets respectively using the same backbone.

==> figures/3-3-Visualization.tex <==
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{figs/triplet_visualization.png}
	\caption{
	Visualization of our generated triplet and corresponding Optical Flow.
    }
	\label{fig:visualization}
\end{figure}

==> figures/4-2-Class-Distribution.tex <==
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{figs/relative_performance.png}
	\caption{
	Class distribution of our proposed method vs Random Init. Each point represent one class average. Abscissa is frame classification while the vertical axis is relative performance of our method over 3D backbone.
	Red line is linear regression result, which indicates our method lead to better result when less rely on context.
    }
	\label{fig:class}
\end{figure}

==> figures/4-3-TSNE-Visualization.tex <==
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{figs/t_sne.png}
	\caption{
	\textbf{T-SNE visualization of learned embedding space of UCF101 but test with videos from the other domain HMDB51.} 
	We random select ten classes from HMDB51 and feed these samples into model with random initialization vs. ours self-supervised pretrain on UCF101.
	These samples become more diverse and easier to be classified even never seen during training.
    }
	\label{fig:tSNE}
\end{figure}

==> tables/4-3-SameDataSet.tex <==
\begin{table}[t]
 \setlength{\belowcaptionskip}{1pt}
    \centering
    {
    \begin{tabular}{lll}
    \toprule
    Self-supervised Pretrain & Finetune & Top-1 \\
    \midrule
    -& UCF101 & 60.3 \\
    UCF101 & UCF101 & \\
    HMDB51 & UCF101 & \\
    Kinetics & UCF101 & \\
    \midrule
    - & HMDB51 & 27.2 \\
    HMDB51&HMDB51& \\
    UCF101&HMDB51&\\
    Kinetics&HMDB51&\\
    \midrule
    -&Kinetics & 70.5 \\
    Kinetics&Kinetics& 73.0 \\
    \bottomrule
    \end{tabular}
    }
    \caption{The performance improvement of self-supervised .}
    \label{tab:performance_improvement}
\end{table}



==> tables/4-6-Semi-supervised.tex <==
\begin{table}
\small
\centering
\begin{tabular}{llll}
\toprule
\bf Method & \bf Architecture & \bf 1\% & \bf 10\% \\
\hline
Supervised baseline & I3D & & \\
Supervised baseline & 3D ResNet-18 & & \\
\midrule
MoCo & I3D & & \\
MoCo & 3D ResNet-18 & & \\
SimCLR & I3D & & \\
SimCLR & 3D ResNet-18 & & \\
\midrule
Ours (Triplet) & I3D &  & \\
Ours (Triplet) & 3D ResNet-18 &  & \\
Ours (Contrastive) & I3D & &  \\
Ours (Contrastive) & 3D ResNet-18 & & \\
\bottomrule
\end{tabular}
\caption{Kinetics accuracy of models trained with few labels.}
\label{tab:semi_super}
\end{table}


